SMCQL: Secure Querying for Federated Databases

People and machines are collecting data at an unprecedented rate. Despite this newfound abundance of data, progress has been slow in sharing it for open science, business, and other data-intensive endeavors. Many such efforts are stymied by privacy concerns and regulatory compliance issues. For example, many hospitals are interested in pooling their medical records for research, but none may disclose arbitrary patient records to researchers or other healthcare providers. In this context we propose the Private Data Network (PDN), a federated database for querying over the collective data of mutually distrustful parties. In a PDN, each member database does not reveal its tuples to its peers nor to the query writer. Instead, the user submits a query to an honest broker that plans and coordinates its execution over multiple private databases using secure multiparty computation (SMC). Here, each database's query execution is oblivious, and its program counters and memory traces are agnostic to the inputs of others. We introduce a framework for executing PDN queries named SMCQL. This system translates SQL statements into SMC primitives to compute query results over the union of its source databases without revealing sensitive information about individual tuples to peer data providers or the honest broker. Only the honest broker and the querier receive the results of a PDN query. For fast, secure query evaluation, we explore a heuristics-driven optimizer that minimizes the PDN's use of secure computation and partitions its query evaluation into scalable slices.

==> optimization/sliced.tex <==
\subsubsection{Partitioning Secure Computation}
\label{sec:sliced}
Now that we have our query plan and have translated the secure operators into garbled circuits, we will examine how we partition the input data of sliced operators for secure processing.  There are several reasons why this slicing is important for high-performance SMC execution.  

First, as described above, sliced operators often have much simpler program logic and thus less depth in their garbled circuits. % when we run in slice mode, we can often generate from a simpler sliced template of an operator.  

Second, slicing reduces the cumulative effect of cascades of operators.  As query trees grow larger, each secure operator's input sizes are a function of that of their children.  For example, say we have two cascading joins and each join input consists of $n$ tuples.  The first oblivious join will produce $n^2$ tuples and the subsequent one will produce an ORAM instance with $n^3$ elements.  When we slice the inputs, we may tame this complexity. 

 Lastly, since  segments identify groups of sliced-alike operators, this further reduces our ORAM-related costs by creating a set of smaller ORAM instances, once per slice value rather than a single large data structure.  Since the ORAM access cost is proportional to the number of tuples in its array, this is a substantial savings.  We will now examine how {\sc \sysname} identifies segments of sliced operators.


%\subsubsection{Slice-Level Planning}
In sliced query execution, we first identify the {\it slice values} that require coordination between parties in a PDN, such as all of the {\em c.\@ diff} patient IDs that appear in both data providers.   We use slice values to bin together tuples that need to be evaluated within the same set of garbled circuits.  We invoke the segment's generated code once per slice value to compute its part of the secure query evaluation.


We first create a composite slice key, the union of the attributes that are slice keys on one or more operators in a segment.   If a slice key contains join predicates, all of the attributes it references are included in the composite key.  This segment key dictates what public values need to be aligned in all of the source data for a slice value to require coordination.  The planner then generates a query listing  the distinct slice values  associated with each attribute in the key. 


If a segment's slice key contains just one attribute, $s_i$, then each party, $p$ probes their database for attribute $s_i$ to produce a list of slice values  $t_{i,p}$ where $p$ may be equal to $A$ or $B$ for Alice or Bob respectively. The parties each report these values via an encrypted connection to the honest broker to prevent leaking information about a party's data distribution. 
 If the segment has a single slice key, $i$, the honest broker finds the slice values for execution as: \[ 
I = t_{i, A} \cap t_{i, B}
\]

We combine these statistics to tell us which slice values need to be computed within SMC.  

If a segment has $k$ slice keys $S = \{s_1, ..., s_k\}$,  we calculate the key values needed for the entire segment as:
\[
I = \bigcap_{i=1}^{k-1}  t_{i, A} \cap  t_{i+1, B}
\]

We identify the possible join matches for attribute $i$ and attribute $i+1$ between Alice and Bob by iterating through the list of slice values associated with each key.  Each secure leaf only computes on tuples with slice values in $I$.   


In addition to identifying fine-grained slice values that will be evaluated together, we also find out which slice values will not require coordination\textendash the {\it slice complement}.  Since we know that any tuples with slice values not in $I$ can be processed without coordination, each party $p$ creates a separate plaintext execution track for the slice complement of table $i$, $t_i$.  The planner determines the slice complement once per secure leaf:
\[
 P_i = t_{i, p} \setminus I
\]
\noindent It is the set complement of $I$.  We put this selection criteria into the filter for the table scans and joins that make up the slice complement.  

To continue our  {\em aspirin count} example, the sliced segment's key is $(d.patient\_id, m.patient\_id)$ and its parent is sliced on the latter attribute.  Thus the planner collects a list of patient ids for each attribute within each party.   It selects patient ids for distributed execution iff a diagnoses.patient\_id appears in Alice and the same patient also appears in Bob's aspirin prescriptions or vice versa.  The sliced join then tests to see if the MI diagnoses happened before or during an encounter when the patient was prescribed aspirin by comparing the private timestamps associated with each event.  In other words, there has to be a potential distributed join match for a slice value to be run with secure execution.   Patient IDs that do not match this criteria for distributed slice execution are evaluated locally on each host in the slice complement.  The complement and the distributed slices are merged into a single ORAM for evaluation in the {\tt COUNT}.  





To summarize, each party prepares one ORAM instance per slice value in $I$ and both parties pass their inputs into a merge to prepare the data for processing in {\sc \sysname}'s generated operators.  In addition, the honest broker generates a plaintext version of each sliced segment for computing over the slice complement, or remaining tuples that do not appear in the intersection set of the slice key over both parties.



==> optimization/smc-rewrites.tex <==
\subsection{Simplifying Secure Computation}
%Physical Query Optimizations
We now examine heuristics that reduce the complexity of our generated SMC code.  These optimizations alter the structure of the code generated by SMC but do not alter the logical flow of data into from plaintext into SMC.   We compile operators with a secure type checker~\cite{liu2014automating}  and delegate to this to prove the security of our generated code.

%\noindent{\bf Sorting} In order to make our generated SMC code perform efficiently, we minimize the random access performed by each operator.
%want to minimize the number of times we access each input tuple.  This reduces the times we pay the high performance penalty associated with each ORAM access. 
%To this end, {\sc \sysname} assigns a {\it secure compute order} to operators that will benefit from sorted inputs.  The sort order enables the engine to compare adjacent tuples for multi-tuple operations.  For example, if we are securely computing a distinct operator, we may evaluate it  faster if the data is already ordered by all of its attributes.  This way we only need to check if neighboring tuples are the same rather than comparing each tuple to all of the ones after it.  %This is primarily aids in the computation of split operators.


%If an operator takes in plaintext data, its unencoded inputs are sorted before we ingest them  into SMC.  Otherwise, if an operator has a conflicting compute order with that of its children, the query planner  inserts a sort between the mismatched operators in the generated code.  %For oblivious sorting we use the bitonic sort algorithm at a cost of O($n\,log^2 n$), where $n$ is the number of array elements.   

%Several relational algebra operators are made faster by sorting their inputs.   Aggregates have a secure compute order of their group-by clause, and this permits us to directly combine partially computed aggregates from multiple hosts.    Likewise, for sorts with multiple sources, we presort and merge the results.   


\noindent{\bf Attribute Trimming}  After each operator, we project out any attributes that are not referenced in its parent or higher ancestors.  We do this by traversing the tree bottom-up, detecting the last time a given attribute or expression is referenced.   This reduces the number of bits in each secure intermediate result making our secure computation simpler and faster.   


%\noindent{\bf Precomputing Filters}  For filters that compare attributes or expressions thereof to literals, we precompute the comparison in plaintext and emit a boolean filter value for SMC.   Thus rather than doing complex comparisons inside SMC, such as $medication\, = \, '\%aspirin\%',$ each data provider computes this expression locally.   We maintain obliviousness by emitting the same number of tuples regardless of whether the filter evaluates true, and the secure query execution nulls out the tuples that do not match the predicate inside SMC.  This dramatically simplifies our SMC code and permits us to support a very broad set of SQL expressions at no additional cost in code complexity or performance.




\noindent{\bf Loop Coalescing}  
To minimize the number of passes we make over the data in a secure query execution, we combine single-tuple operators with neighboring ones.   We push {\it up} filters to their parent operators so that both may execute in a single loop.  In addition, {\sc \sysname}  evaluate projections within the body of its child operator. More details on this are in Section~\ref{sec:code-gen}.

%Recall that if a filter references sensitive data, we need to run it obliviously.   Run alone, this means that the filter would need to make a pass over all of the tuples it received, emitting the same number of tuples in output that it received, where some of them may be null.   Owing to its secure compute order,  every operator, except sort and join, makes a single linear scan over its inputs.  We push the filter up to the first parent operator that has multi-tuple operations  to avoid performing extra iterations over the data. Likewise, performing projections within the body of their source operator reduces the number of times we need to do expensive reads and writes on the data.  


==> pdns.tex <==
\section{Private Data Networks}
\label{sec:pdns} 
We now introduce the architecture within which {\sc \sysname} runs queries over mutually distrustful parties. Private Data Networks, or PDNs, are a generalization of federated databases that enable two or more databases to work together to compute a query without sharing their data with one another. %To accomplish this, the framework needs a way to reason about the security requirements of a PDN and the relational algebra used in a query.

%\subsection{Architecture}

Our prototype's architecture is shown in Figure~\ref{fig:architecture-diagram}.  The {\it honest broker} is the entry and exit point of the PDN, and it is a trusted, neutral federator that plans and coordinates query evaluation over its data providers.  In the figure, Alice and Bob represent the two data providers who do not trust one another in the PDN.  After receiving a plaintext query from the user, the honest broker rewrites it into a secure query plan that contains a mix of plaintext and SMC execution steps.  %This query plan is comprised of a series of plaintext and secure execution steps that, when taken together, compute a given SQL statement.

To set up a PDN, the data providers begin with a shared set of table definitions. This schema is annotated with the level of protection required for each attribute in the tables.  In addition, the configuration denotes whether a table is replicated or partitioned among members.  For matching identifiers, such as patient IDs in HealthLNK, the honest broker works with the data providers to carry out secure record linkage~\cite{al2005blocking, kho2015linkage,lazrig2015privacy}.


%A PDN query execution begins when a  user submits a SQL statement to the honest broker.  The broker uses a regular database with the PDN's table definitions to compile the SQL statement into a directed acyclic graph (DAG) of database operators. Using this query tree, the planner automatically generates a query plan containing a mix of plaintext and SMC execution.  It uses the annotated schema to determine the level of security needed for each node in the operator tree based on the attributes it computes on and how it accesses them.

A PDN query execution begins when a  user submits a SQL statement to the honest broker.  The broker uses a regular database with the PDN's table definitions to compile the SQL statement into a set of steps to be executed either in plaintext in the member databases or among PDN data providers using SMC.  Once this query plan is generated, the honest broker sends a copy of it to both Alice and Bob.  For each secure step Alice generates the garbled circuits needed for its computation, and she passes them to Bob for evaluation.  After the parties finish computing all steps in the plan, Alice and Bob return their respective garbled circuit outputs to the honest broker, who combines them to reveal the plaintext query results. The honest broker then ships this output to the user.

\begin{figure} [t]
\centering
\includegraphics[width=0.5\textwidth]{figures/architecture-diagram} %natwidth=673,natheight=441
\caption{Architecture of a two-party private data network.}
\label{fig:architecture-diagram}
\vspace{-5mm}
\end{figure}


% Example app was here


Looking at our architecture in Figure~\ref{fig:architecture-diagram}, we see how CAPriCORN would be configured as a PDN. Alice and Bob are two healthcare sites, each containing a database with PHI and data that does not require protection. The honest broker is a trusted coordinator that takes a plaintext query from the user, rewrites it into a {\sc \sysname} query plan, and passes that query plan to two or more hospitals.  From here, the two parties generate and evaluate garbled circuits, which are then returned to the honest broker. The honest broker combines the result shares to reveal the plaintext results that it sends to the user.  This architecture distributes the computation among Alice and Bob, decreasing the maximum load on any one hospital in the network. For CDRNs, this distributed computation is extremely important. If a PDN performs most or all of its computation within the honest broker, this system will not scale to the large number of users who wish to issue queries to consortium members.  

